Satellite Safe Margin: Fast solutions for Conjunction Analysis

The amount of debris in orbit has increased significantly over the years. With the recent growth of interest in space exploration, conjunction assessment has become a central issue. One important metric to evaluate conjunction risk is the miss distance. However, this metric does not intrinsically take into account uncertainty distributions. Some work has been developed to consider the uncertainty associated with the position of the orbiting objects, in particular, to know if these uncertainty distributions overlap (e.g., ellipsoids when considering Gaussian distributions). With this work, we present fast solutions to not only check if the ellipsoids overlap but to compute the distance between them, which we call margin. We present two fast solution methods for two different paradigms: when the best-known data from both objects can be centralized (e.g., debris-satellite conjunctions) and when the most precise covariances cannot be shared (conjunctions of satellites owned by different operators). Our methods are both accurate and fast, being able to process 15,000 conjunctions per minute with the centralized solution and approximately 490 conjunctions per minute with the distributed solution.

==> Files/background.tex <==
\section{Background}

In this section, we present the general formulation of the two first-order optimization methods used in this work, the Frank-Wolfe Algorithm and the Fast Iterative Shrinkage-Thresholding Algorithm, as well as the analytical method for estimating the distance between ellipses proposed by Rimon and Boyd.

\subsection{Frank-Wolfe Algorithm}

\noindent The Frank-Wolfe (FW) Algorithm \cite{frank1956algorithm} is a first-order method that aims to solve the optimization problem

\begin{equation}
    \label{eq:frank-wolfe-problem}
    \begin{aligned}
        &\underset{x \in \mathcal{D}}{\mbox{minimize}} \quad f(x)
    \end{aligned}
\end{equation}
%
such that $\mathcal{D}$ is a compact and convex set, and $f: \mathcal{D} \mapsto \mathbb{R}$ is a convex and differentiable function. At each iteration, the algorithm aims to minimize a linear approximation of the objective function over the same domain $\mathcal{D}$ of the original problem. In the constrained optimization setting, this method stands out for not needing a projection or proximal step to remain feasible.

The original Frank-Wolfe algorithm is systematized in Algorithm~\ref{alg:original-frank-wolfe}. At each iteration, after the minimization of the linear approximation, the next iteration moves in the direction of the computed minimizer with step size $\alpha = \frac{2}{k+2}$ at the $k$-th iteration.

\begin{algorithm}[h!]
\caption{Frank-Wolfe}
\label{alg:original-frank-wolfe}
\begin{algorithmic}
\Require{$x \in \mathcal{D}$}
\State $x^0 \gets x$

\For{$k = 0,...,n$}
    \State $s^k \gets \underset{s \in \mathcal{D}}{\arg\min} \ s^T \nabla f(x^k)$
    \State $\alpha \gets \frac{2}{k+2}$
    \State $x^{k+1} \gets x^k + \alpha (s^k - x^k)$

\EndFor
\end{algorithmic}
\end{algorithm}
%
The algorithm has a convergence rate for the objective of $O\left(\frac{1}{k}\right)$ and has regained relevance in several areas given its low implementation cost and good scalability. Based on the original algorithm, new variants of this algorithm have been presented and analyzed with relevant features to increase the progress in each iteration \cite{jaggi2013revisiting,pedregosa2020linearly,lacoste2015global,dvurechensky2022generalized,liu2016efficient,guelat1986some}. 

We will analyze, in more detail, one of these variants, which we will use to solve our problem. Instead of using the predefined value of $\alpha = \frac{2}{k+2}$, we can find the best step size for each particular iteration through line search. So $\alpha$ can be chosen as

\begin{equation}
    \label{eq:frank-wolfe-line-search-alpha}
    \begin{aligned}
        \alpha = \underset{\alpha \in [0,1]}{\arg\min} \ f(x^k + \alpha (s^k - x^k)).
    \end{aligned}
\end{equation}
%
Therefore, the next iteration is the best point belonging to the line segment between the current iteration $x^k$ and $s$. A formal definition of the Frank-Wolfe algorithm with step-size line search can be found in Algorithm~\ref{alg:line-search-frank-wolfe}.

\begin{algorithm}[h!]
\caption{Frank-Wolfe with Line Search for step size $\alpha$}
\label{alg:line-search-frank-wolfe}
\begin{algorithmic}
\Require{$x \in \mathcal{D}$}
\State $x^0 \gets x$

\For{$k = 0,...,n$}
    \State $s^k \gets \underset{s \in \mathcal{D}}{\arg\min} \ s^T \nabla f(x^k)$
    \State $\alpha \gets \underset{\alpha \in [0,1]}{\arg\min} \ f(x^k + \alpha (s^k - x^k))$
    \State $x^{k+1} \gets x^k + \alpha (s^k - x^k)$
\EndFor
\end{algorithmic}
\end{algorithm}
%
\subsection{Fast Iterative Shrinkage-Thresholding Algorithm (FISTA)}

Consider the general problem formulation

\begin{equation}
    \label{eq:fista-general-problem-formulation}
    \begin{aligned}
        &\underset{x \in \mathbb{R}^n}{\mbox{minimize}} \quad f(x) + g(x)
    \end{aligned}
\end{equation}
%
with the following assumptions:

\begin{itemize}
    \item[$\bullet$] $g: \mathbb{R}^n \rightarrow \mathbb{R}$ is convex (possibly non-smooth);
    \item[$\bullet$] $f: \mathbb{R}^n \rightarrow \mathbb{R}$ is proper and closed, dom($f$) is convex, dom($g$) $\subseteq$ int(dom($f$)), and $f$ is $L_f$-smooth over int(dom($f$));
    \item[$\bullet$] The optimal set of problem~\eqref{eq:fista-general-problem-formulation} is nonempty.
\end{itemize}
%
A simple way to minimize the function $f$, and with low computational cost, is to use the gradient algorithm whose iteration step is defined as

\begin{equation}
    \label{eq:iteration-step}
    \begin{aligned}
        x^{k+1} = x^k - \frac{1}{L_k} \nabla f(x^k),
    \end{aligned}
\end{equation}
%
where $x^k$ and $L_k$ denotes the values of $x$ and $L$ at iteration $k$, with $\frac{1}{L_k} > 0$ defining the step-size. Since the $g$ function can possibly be non-smooth, the proximal operator is normally used, which can be defined as

\begin{equation}
    \label{eq:proximal-operator}
    \begin{aligned}
        \mbox{prox}_g(x) = \underset{u}{\arg\min} \ \left\{g(u) + \frac{1}{2} \|u - x\|^2\right\}.
    \end{aligned}
\end{equation}
%
The idea of the proximal operator is, given a point $x$, we aim to find the closest point to $x$ that minimizes the function $g$. When $g$ is properly closed and convex, $\mbox{prox}_g (\cdot)$ exists and is unique \cite{beck2017first}. 

Let us rewrite update step in~\eqref{eq:iteration-step} as 

\begin{equation}
    \label{eq:rewritten-iteration-step}
    \begin{aligned}
        x^{k+1} = \underset{x}{\mbox{argmin}} \left\{ f(x^k) + \nabla f(x^k)^T (x - x^k) + \frac{L_k}{2} \|x - x^k\|^2 \right\}.
    \end{aligned}
\end{equation}
%
The next iteration is the minimizer of the sum of the linearization of $f$ around the current iteration plus a quadratic proximal term. We can generalize this idea to be the minimizer of the sum of the linearization of $f$ around the current iteration plus a quadratic proximal term plus the proximal operator $g$ as

\begin{equation}
    \label{eq:rewritten-g-iteration-step}
    \begin{aligned}
        x^{k+1} = \underset{x}{\mbox{argmin}} \left\{ f(x^k) + \nabla f(x^k)^T (x - x^k) + \frac{L_k}{2} \|x - x^k\|^2 + g(x) \right\}.
    \end{aligned}
\end{equation}
%
After some manipulation, we obtain

\begin{equation}
    \label{eq:rewritten-g-iteration-step-reformulation}
    \begin{aligned}
        x^{k+1} = \underset{x}{\mbox{argmin}} \left\{ \frac{1}{L_k} g(x) + \frac{1}{2} \left\|x - \left(x^k - \frac{1}{L_k} \nabla f(x^k)\right)\right\|^2 \right\}.
    \end{aligned}
\end{equation}
%
By definition of the proximal operator (as in~\eqref{eq:proximal-operator}), this is equivalent to

\begin{equation}
    \label{eq:iteration-step-prox-operator}
    \begin{aligned}
        x^{k+1} =\mbox{prox}_{\frac{1}{L_k} g}\left(x^k - \frac{1}{L_k} \nabla f(x^k)\right).
    \end{aligned}
\end{equation}
%
Thus, the proximal gradient method solves problems with the same shape as in~\eqref{eq:fista-general-problem-formulation}, whose iteration step is defined as in~\eqref{eq:iteration-step-prox-operator}. With this we can design what is called the Proximal Gradient method: pick $x^0 \in \mbox{int(dom}(f))$ and iteratively apply the update step~\eqref{eq:iteration-step-prox-operator}.

Analyzing some particular cases, when $g \equiv 0$, then the update step reduces to the gradient step as described in~\eqref{eq:iteration-step}. When $g = \delta_C$, where $\delta_C$ is the indicator function of the set $C$, written as

\begin{equation}
    \label{eq:general-indicator-function}
    \begin{aligned}
        \delta_C(x) = \begin{cases}
        0 & \quad \mbox{if } x \in C \\
        +\infty & \quad \mbox{otherwise}
        \end{cases}
    \end{aligned}
\end{equation}
%
such that $C$ is a nonempty closed and convex set, then the proximal operator becomes the orthogonal projection operator, $P_C$, which projects a point to the set C \cite{beck2017first}.

However, the proximal gradient method achieves a rate of convergence of $O\left(\frac{1}{k}\right)$. \citeauthor{nesterov1983method} presented a method based on a multistep scheme with a rate of convergence of $O\left(\frac{1}{k^2}\right)$ for this class of problems and proved that this rate of convergence is optimal and cannot be improved \cite{nesterov1983method}. \citeauthor{beck2009fast} present the Fast Iterative Shrinkage-Thresholding Algorithm (FISTA) \cite{beck2009fast}, which has a variant of the multistep scheme that achieves the same theoretical optimal convergence rate. A description of the FISTA algorithm can be found in Algorithm~\ref{alg:fista}.

\begin{algorithm}[h!]
\caption{Fast Iterative Shrinkage-Thresholding Algorithm (FISTA)}
\label{alg:fista}
\begin{algorithmic}
\Require{$p \in \mbox{int(dom}(f))$, $f$ and $g$ with assumptions made for Problem~\eqref{eq:fista-general-problem-formulation}}
\State $x^0 \gets p$
\State $y^0 \gets x^0$
\State $t^0 \gets 1$

\For{$k = 0,...,n$}
    \State pick $L_k$ as Lipschitz constant of the gradient of the loss ($L_f$) or value found by backtracking
    \State $x^{k+1} \gets \mbox{prox}_{\frac{1}{L_k}g}(y^k - \frac{1}{L_k} \nabla f(y^k))$
    \State $t^{k+1} \gets \frac{1 + \sqrt{1 + 4 (t^k)^2}}{2}$
    \State $y^{k+1} \gets x^{k+1} + \left(\frac{t^k - 1}{t^{k+1}}\right) (x^{k+1} - x^k)$
\EndFor
\end{algorithmic}
\end{algorithm}
%
The main difference is that the proximal operator is not applied on the previous point $x^{k-1}$. Instead, it is applied on $y^k$ which is a specific linear combination of the previous two iterations, $x^{k-1}$ and $x^{k-2}$ \cite{beck2009fast}. This multistep scheme allows us to obtain the optimal convergence rate of $O\left(\frac{1}{k^2}\right)$. The choice of stepsize $\frac{1}{L_k}$ can be done in two ways:

\paragraph*{Constant stepsize:}

Remembering that the function $f$ is $L_f$-smooth, we can choose $L_k$ as the Lipschitz constant, $L_f$, of the gradient of the function $f$, so $L_k = L_f$ for all $k$.

\paragraph*{Backtracking procedure:}

Choose $s > 0$ and $\eta > 1$. Define $L_{-1} = s$. At iteration $k$ $(k \geq 0)$, we choose $L_k$ as follows: first, set $L_k = L_{k-1}$. While

\begin{equation}
    \begin{aligned}
        f(T_{L_k}(y^k)) > f(y^k) + \nabla f(y^k)^T (T_{L_k}(y^k) - y_k) + \frac{L_k}{2} \|T_{L_k}(y^k) - y^k\|^2,
    \end{aligned}
\end{equation}
%
we set $L_k = \eta L_k$, such that

\begin{equation}
    \begin{aligned}
        T_{L_k}(x) = prox_{\frac{1}{L_k} g}(x - \frac{1}{L_k} \nabla f(x)).
    \end{aligned}
\end{equation}
%

\subsection{Distance Estimation between Ellipsoids}
\label{sec:distance-estimation}

This method was presented by \citeauthor{rimon1997obstacle} to detect obstacle collision \cite{rimon1997obstacle} . The authors simplify the shape of objects by resorting to minimum-volume enclosing ellipsoids and perform an eigenvalue-based technique to estimate the distance between the ellipses.

First, we see how to calculate the minimum Euclidean distance of a point $x_0 \in \mathbb{R}^n$ to an n-ellipsoid $\xi^n(a, A) = \left\{ p \in \mathbb{R}^n : (p - a)^T A (p - a) \leq 1 \right\}$. For this, we consider that $x_0$ lies outside $\xi^n(a, A)$ and that it is at the origin of $\mathbb{R}^n$. Therefore, we intend to solve the following optimization problem

\begin{equation}
    \label{eq:distance-optimization-problem}
    \begin{aligned}
        &\mbox{Minimize} \quad \phi(X) = \| x \| \\
        &\mbox{subject to} \quad (x - a)^T A (x - a) = 1.
    \end{aligned}
\end{equation}
%
The solution $x^*$ must satisfy the following Lagrange multiplier rule: $x^* = \lambda A (x^* - a)$, for some scalar $\lambda$. Developing this expression we have

\begin{equation}
    \label{eq:langragian-rule}
    \begin{aligned}
        &x^* = \lambda A (x^* - a) \Leftrightarrow \\
        &x^* = \lambda [\lambda A - I]^{-1} Aa \Leftrightarrow \\
        &x^* - a = [\lambda A - I]^{-1} a,
    \end{aligned}
\end{equation}
%
and substituting for $x^* - a$ in the constraint of the problem \eqref{eq:distance-optimization-problem}, we have $\Tilde{a}^T [A^{-1} - \lambda I]^{-2}\Tilde{a} = 1$, where $\Tilde{a} = A^{-\frac{1}{2}}a$. The minimal root $\lambda$ which corresponds to $x^*$ can be computed as an eigenvalue problem. We start by defining two new variables:

\begin{equation}
    \label{eq:eigenvalue-problem-variables}
    \begin{aligned}
        w \coloneqq [A^{-1} - \lambda I]^{-2}\Tilde{a} \quad \mbox{and} \quad z \coloneqq [A^{-1} - \lambda I]^{-2}\Tilde{a}.
    \end{aligned}
\end{equation}
%
With this, we can express the above equations in terms of $\lambda$, $w$ and $z$ and we get the following equations:

\begin{equation}
    \label{eq:eigenvalue-problem-equations}
    \begin{cases}
        &\Tilde{a}^T w = 1 \\
        &[A^{-1} - \lambda I]z = \Tilde{a} \\
        &[A^{-1} - \lambda I]w - z = 0
    \end{cases} \Leftrightarrow
    \begin{cases}
        &\Tilde{a}^T w = 1 \\
        &[A^{-1} - \lambda I]z = [\Tilde{a}\Tilde{a}^T] w \\
        &[A^{-1} - \lambda I]w - z = 0.
    \end{cases}
\end{equation}
%
Combining the second and third equation, we end up with the following eigenvalue problem:

\begin{equation}
    \label{eigenvalue-problem-formulation}
    \begin{aligned}
        \begin{bmatrix}
            A^{-1} & -I \\
            -\Tilde{a}\Tilde{a}^T & A^{-1}
        \end{bmatrix}
        \begin{pmatrix}
            w \\
            z
        \end{pmatrix} = \lambda
        \begin{pmatrix}
            w \\
            z
        \end{pmatrix},
    \end{aligned}
\end{equation}
%
so, let $M$ be the $2n \times 2n$ matrix in (\ref{eigenvalue-problem-formulation}) and $\lambda_{\min}(M)$ its minimal eigenvalue, we have that the distance between $x$ and $\xi^n(a, A)$) is $\| x - x^* \|$, where $x^* = \lambda_{\min}(M) [\lambda_{\min}(M) A - I]^{-1} Aa$.

Now, based on the distance between a point and an ellipsoid, we can compute the distance estimate between two $n$-ellipsoids, $\xi_1 = \xi^n(b, B)$ and $\xi_2 = \xi^n(c, C)$. We start by computing $x^* \in \xi_2$ at which the ellipsoidal level surfaces surrounding $\xi_1$ first touch $\xi_2$. Then we compute $y^* \in \xi_1$ which is the closest to $x^*$. The distance estimate is then margin($\xi_1$, $\xi_2$) = $\| x^* - y^* \|$. The authors summarize this computation in the following proposition:

\begin{proposition}
\label{prop:margin-estimation}
Given two $n$-ellipsoids $\xi_1 = \xi^n(b, B)$ and $\xi_2 = \xi^n(c, C)$, the point $x^* \in \xi_2$ is $x^* = b + \lambda_1 B^{-\frac{1}{2}} [\lambda_1 I - \Tilde{C}]^{-1} \bar{c}$, where $\Tilde{C} = \overline{C} \,^{-1}$ and $\lambda_1$ is the minimal eigenvalue of the $2n \times 2n$ matrix

\begin{equation}
    \label{eq:min-eigenvalue-1}
    \begin{bmatrix}
            \Tilde{C} & -I \\
            -\Tilde{c}\Tilde{c}^T & \Tilde{C}
        \end{bmatrix}
\end{equation}
%
such that $\overline{C} = B^{-\frac{1}{2}} C B^{-\frac{1}{2}}$ and $\Tilde{c} = \overline{C} \,^{-\frac{1}{2}} B^{\frac{1}{2}}(c - b)$.

The point $y^* \in \xi_1$ is $y^* = x^* + \mu_1 [\mu_1 I - \Tilde{B}]^{-1} b$, where $\Tilde{B} = B^{-1}$ and $\mu_1$ is the minimal eigenvalue of the $2n \times 2n$ matrix

\begin{equation}
    \label{eq:min-eigenvalue-2}
    \begin{bmatrix}
            \Tilde{B} & -I \\
            -\Tilde{b}\Tilde{b}^T & \Tilde{B}
        \end{bmatrix}
\end{equation}
%
such that $\Tilde{b} = \overline{B} \,^{-\frac{1}{2}} b$. The distance estimate margin($\xi_1$, $\xi_2$) = $\| x^* - y^* \|$, is positive when $\xi_1$ and $\xi_2$ are disjoint, and zero when $\xi_1$ and $\xi_2$ touch such that their interiors are disjoint.

\end{proposition}
